Learning State Representations in Complex Systems with Multimodal Data

Representation learning becomes especially important for complex systems with multimodal data sources such as cameras or sensors. Recent advances in reinforcement learning and optimal control make it possible to design control algorithms on these latent representations, but the field still lacks a large-scale standard dataset for unified comparison. In this work, we present a large-scale dataset and evaluation framework for representation learning for the complex task of landing an airplane. We implement and compare several approaches to representation learning on this dataset in terms of the quality of simple supervised learning tasks and disentanglement scores. The resulting representations can be used for further tasks such as anomaly detection, optimal control, model-based reinforcement learning, and other applications.

==> airports_benchmarks.tex <==
\toprule
{} &                   city & country & iata &  icao &                                               name &  split \\
\midrule
0  &               Kingston &      CA &  YGK &  CYGK &                     Kingston Norman Rogers Airport &  train \\
1  &               Montreal &      CA &  YMX &  CYMX &           Montreal International (Mirabel) Airport &  train \\
2  &                Trenton &      CA &  YTR &  CYTR &                                        CFB Trenton &  train \\
3  &              Maiduguri &      NG &  MIU &  DNMA &                    Maiduguri International Airport &  train \\
4  &                 Ostend &      BE &  OST &  EBOS &                Ostend-Bruges International Airport &  train \\
5  &        Friedrichshafen &      DE &  FDH &  EDNY &                            Friedrichshafen Airport &  train \\
6  &                Kittila &      FI &  KTT &  EFKT &                                    Kittila Airport &  train \\
7  &                 Dublin &      IE &  DUB &  EIDW &                                     Dublin Airport &  train \\
8  &                   Oslo &      NO &  OSL &  ENGM &                            Oslo Gardermoen Airport &  train \\
9  &              Stavanger &      NO &  SVG &  ENZV &                             Stavanger Airport Sola &  train \\
10 &                 Luanda &      AO &  LAD &  FNLU &                        Quatro De Fevereiro Airport &  train \\
11 &                 Maputo &      MZ &  MPM &  FQMA &                                     Maputo Airport &  train \\
12 &               Blantyre &      MW &  BLZ &  FWCL &                      Chileka International Airport &  train \\
13 &                 Agadir &      MA &  AGA &  GMAD &                                 Al Massira Airport &  train \\
14 &             Casablanca &      MA &  CMN &  GMMN &                   Mohammed V International Airport &  train \\
15 &                 Assiut &      EG &  ATZ &  HEAT &                       Assiut International Airport &  train \\
16 &          Dar es Salaam &      TZ &  DAR &  HTDA &    Mwalimu Julius K. Nyerere International Airport &  train \\
17 &              Watertown &      US &  ART &  KART &                    Watertown International Airport &  train \\
18 &         Elmira/Corning &      US &  ELM &  KELM &                    Elmira Corning Regional Airport &  train \\
19 &               New York &      US &  JFK &  KJFK &               John F Kennedy International Airport &  train \\
20 &                  Paris &      FR &  ORY &  LFPO &                                 Paris-Orly Airport &  train \\
21 &  Luxeuil/Saint-Sauveur &      FR &      &  LFSX &            Luxeuil-Saint-Sauveur (BA 116) Air Base &  train \\
22 &                        &      CH &      &  LSME &                                      Emmen Airport &  train \\
23 &             Altenrhein &      CH &  ACH &  LSZR &                       St Gallen Altenrhein Airport &  train \\
24 &         Guatemala City &      GT &  GUA &  MGGT &                                  La Aurora Airport &  train \\
25 &                Tijuana &      MX &  TIJ &  MMTJ &  General Abelardo L. Rodriguez International Ai... &  train \\
26 &                Holguin &      CU &  HOG &  MUHG &                   Frank Pais International Airport &  train \\
27 &                 Ezeiza &      AR &  EZE &  SAEZ &           Ministro Pistarini International Airport &  train \\
28 &         Rio De Janeiro &      BR &  GIG &  SBGL &  Galeao - Antonio Carlos Jobim International Ai... &  train \\
29 &                  Sochi &      RU &  AER &  URSS &                        Sochi International Airport &  train \\
30 &             Copenhagen &      DK &  RKE &  EKRK &                        Copenhagen Roskilde Airport &    val \\
31 &   Stockholm / Nykoping &      SE &  NYO &  ESKN &                          Stockholm Skavsta Airport &    val \\
32 &       Lanzarote Island &      ES &  ACE &  GCRR &                                  Lanzarote Airport &    val \\
33 &                  Oujda &      MA &  OUD &  GMFO &                                     Angads Airport &    val \\
34 &              Marrakech &      MA &  RAK &  GMMX &                                     Menara Airport &    val \\
35 &                        &      MA &  TTU &  GMTN &                                Saniat Rmel Airport &    val \\
36 &                Massena &      US &  MSS &  KMSS &               Massena International Richards Field &    val \\
37 &       Epinal/Mirecourt &      FR &  EPL &  LFSG &                           Epinal-Mirecourt Airport &    val \\
38 &              Sarmellek &      HU &  SOB &  LHSM &                    Sarmellek International Airport &    val \\
39 &                  Milan &      IT &  MXP &  LIMC &                     Malpensa International Airport &    val \\
40 &               Salzburg &      AT &  SZG &  LOWS &                                   Salzburg Airport &    val \\
41 &                 Geneva &      CH &  GVA &  LSGG &              Geneva Cointrin International Airport &    val \\
42 &                 Zurich &      CH &      &  LSMD &                                  Dubendorf Airport &    val \\
43 &                   Bern &      CH &  BRN &  LSZB &                                  Bern Belp Airport &    val \\
44 &             San Benito &      GT &  FRS &  MGTK &                   Mundo Maya International Airport &    val \\
45 &               Freeport &      BS &  FPO &  MYGF &                 Grand Bahama International Airport &    val \\
\bottomrule

==> airports_encoder_train.tex <==
\toprule
{} &                       city & country & iata &  icao &                                         name &  split \\
\midrule
0  &                  Florennes &      BE &      &  EBFS &                           Florennes Air Base &  train \\
1  &                     Berlin &      DE &  SXF &  EDDB &      Berlin-Schonefeld International Airport &  train \\
2  &                   Helsinki &      FI &  HEL &  EFHK &                      Helsinki Vantaa Airport &  train \\
3  &               Saint Helier &      JE &  JER &  EGJJ &                               Jersey Airport &  train \\
4  &                      Leeds &      GB &  LBA &  EGNM &                       Leeds Bradford Airport &  train \\
5  &                  Amsterdam &      NL &  AMS &  EHAM &                   Amsterdam Airport Schiphol &  train \\
6  &                     Evenes &      NO &  EVE &  ENEV &                Harstad/Narvik Airport Evenes &  train \\
7  &                     Tromso &      NO &  TOS &  ENTC &                               Tromso Airport &  train \\
8  &                       Torp &      NO &  TRF &  ENTO &                      Sandefjord Airport Torp &  train \\
9  &                      Visby &      SE &  VBY &  ESSV &                                Visby Airport &  train \\
10 &                   Ramstein &      DE &  RMS &  ETAR &                            Ramstein Air Base &  train \\
11 &                 Hoedspruit &      ZA &  HDS &  FAHS &            Hoedspruit Air Force Base Airport &  train \\
12 &                 Mpumalanga &      ZA &  MQP &  FAKN &      Kruger Mpumalanga International Airport &  train \\
13 &  Louis Trichardt Southwest &      ZA &      &  FALM &               Makhado Air Force Base Airport &  train \\
14 &                  N'Djamena &      TD &  NDJ &  FTTJ &              N'Djamena International Airport &  train \\
15 &             Victoria Falls &      ZW &  VFA &  FVFA &         Victoria Falls International Airport &  train \\
16 &       Fuerteventura Island &      ES &  FUE &  GCFV &                        Fuerteventura Airport &  train \\
17 &        Gran Canaria Island &      ES &  LPA &  GCLP &                         Gran Canaria Airport &  train \\
18 &            Tenerife Island &      ES &  TFN &  GCXO &                       Tenerife Norte Airport &  train \\
19 &                        Fes &      MA &  FEZ &  GMFF &                                Saiss Airport &  train \\
20 &                      Rabat &      MA &  RBA &  GMME &                           Rabat-Sale Airport &  train \\
21 &                      Nador &      MA &  NDR &  GMMW &                  Nador International Airport &  train \\
22 &                 Nouakchott &      MR &  NKC &  GQNN &             Nouakchott International Airport &  train \\
23 &                Addis Ababa &      ET &  ADD &  HAAB &                   Bole International Airport &  train \\
24 &                 Alexandria &      EG &  HBE &  HEBA &           Borg El Arab International Airport &  train \\
25 &                      Cairo &      EG &  CAI &  HECA &                  Cairo International Airport &  train \\
26 &                 Port Sudan &      SD &  PZU &  HSPN &         Port Sudan New International Airport &  train \\
27 &                   Carlsbad &      US &      &  KCRQ &                   Mc Clellan-Palomar Airport &  train \\
28 &               White Plains &      US &  HPN &  KHPN &                   Westchester County Airport &  train \\
29 &                 Monticello &      US &      &  KMSV &        Sullivan County International Airport &  train \\
30 &                      Provo &      US &      &  KPVU &                      Provo Municipal Airport &  train \\
31 &                  Rochester &      US &  ROC &  KROC &      Greater Rochester International Airport &  train \\
32 &             Salt Lake City &      US &  SLC &  KSLC &         Salt Lake City International Airport &  train \\
33 &                  Santa Ana &      US &  SNA &  KSNA &     John Wayne Airport-Orange County Airport &  train \\
34 &                   Torrance &      US &      &  KTOA &                              Zamperini Field &  train \\
35 &                  Barcelona &      ES &  BCN &  LEBL &              Barcelona International Airport &  train \\
36 &             Annecy/Meythet &      FR &  NCY &  LFLP &       Annecy-Haute-Savoie-Mont Blanc Airport &  train \\
37 &                     Athens &      GR &  ATH &  LGAV &  Eleftherios Venizelos International Airport &  train \\
38 &                   Budapest &      HU &  BUD &  LHBP &  Budapest Listz Ferenc international Airport &  train \\
39 &                     Prague &      CZ &  PRG &  LKPR &                 Ruzyne International Airport &  train \\
40 &                            &      CH &      &  LSMP &                              Payerne Airport &  train \\
41 &                     Zurich &      CH &  ZRH &  LSZH &                               Zurich Airport &  train \\
42 &                    Tocumen &      PA &  PTY &  MPTO &                Tocumen International Airport &  train \\
43 &                Santa Clara &      SV &  SAL &  MSLP &            El Salvador International Airport &  train \\
44 &                     Nassau &      BS &  NAS &  MYNN &        Lynden Pindling International Airport &  train \\
45 &                Belize City &      BZ &  BZE &  MZBZ &   Philip S. W. Goldson International Airport &  train \\
46 &                      Tokyo &      JP &  NRT &  RJAA &                 Narita International Airport &  train \\
47 &                    Omitama &      JP &  IBR &  RJAH &                              Hyakuri Airport &  train \\
48 &                Resistencia &      AR &  RES &  SARE &            Resistencia International Airport &  train \\
49 &             St. Petersburg &      RU &  LED &  ULLI &                              Pulkovo Airport &  train \\
50 &                      Liege &      BE &  LGG &  EBLG &                                Liege Airport &    val \\
51 &                    Tallinn &      EE &  TLL &  EETN &                              Tallinn Airport &    val \\
52 &                    Vilnius &      LT &  VNO &  EYVI &                Vilnius International Airport &    val \\
53 &              Potgietersrus &      ZA &  PTG &  FAPP &              Polokwane International Airport &    val \\
54 &                     Bissau &      GW &  OXB &  GGOV &         Osvaldo Vieira International Airport &    val \\
55 &                   Monrovia &      LR &  ROB &  GLRB &                Roberts International Airport &    val \\
56 &                 Ouarzazate &      MA &  OZZ &  GMMZ &                           Ouarzazate Airport &    val \\
57 &                     Arusha &      TZ &  JRO &  HTKJ &            Kilimanjaro International Airport &    val \\
58 &                 Binghamton &      US &  BGM &  KBGM &        Greater Binghamton/Edwin A Link field &    val \\
59 &                Los Angeles &      US &  LAX &  KLAX &            Los Angeles International Airport &    val \\
60 &                 Montgomery &      US &      &  KMGJ &                        Orange County Airport &    val \\
61 &                   Newburgh &      US &  SWF &  KSWF &                Stewart International Airport &    val \\
62 &                       Nice &      FR &  NCE &  LFMN &                     Nice-Cote d'Azur Airport &    val \\
63 &                   Elefsina &      GR &      &  LGEL &                              Elefsis Airport &    val \\
64 &                   Santiago &      DO &  STI &  MDST &                  Cibao International Airport &    val \\
65 &             Port-au-Prince &      HT &  PAP &  MTPP &   Toussaint Louverture International Airport &    val \\
66 &                 Corrientes &      AR &  CNQ &  SARC &                           Corrientes Airport &    val \\
\bottomrule
